New effective theories of gravitation and their phenomenological consequences

This thesis focuses on modifications on Einstein's theory of General Relativity, which could explain the current problems in gravitation and cosmology. More specifically, modifications of the affine structure of the spacetime, which is the structure that tells us how to perform derivatives, are studied. These theories appear when imposing that the system must be invariant under the action of the local Poincar\'e group. Within these theories, their stability, the conditions for the appearance of singularities, the movement of fermions, and if it is possible to find different Black Hole solutions than in Einstein's theory, is explored. Moreover, a non-local extension of the mentioned modification is proposed, which can make the theory free of instabilities and singularities at the linear limit.

==> Other_frame_field_equations.tex <==
\item Variations with respect to the metric (or \emph{Einstein Equations}):
\begin{equation}
\frac{\delta S}{\delta g^{\mu\nu}}=0\Longrightarrow\frac{\delta\mathcal{L}}{\delta g^{\mu\nu}}-\frac{1}{2}g_{\mu\nu}\mathcal{L}=0.
\end{equation}
Hence we have
\begin{eqnarray}
\label{biscalar:Einstein}
\mathring{G}_{\mu\nu}&=&-\frac{72M_{S}^{2}\left(\chi\right)}{A\left(\chi,\phi\right)\chi}\left(\partial_{\mu}\chi\partial_{\nu}\chi-\frac{1}{2}g_{\mu\nu}\partial_{\rho}\chi\partial^{\rho}\chi\right)+\frac{1}{\chi}\left(\mathring{\nabla}_{\mu}\mathring{\nabla}_{\nu}\chi-g_{\mu\nu}\Box\chi\right)
\nonumber
\\
&&-\frac{72\alpha^{2}M_{T}^{2}\left(\chi\right)}{A\left(\chi,\phi\right)\chi}\left(\partial_{\mu}\phi\partial_{\nu}\phi-\frac{1}{2}g_{\mu\nu}\partial_{\rho}\phi\partial^{\rho}\phi\right)
\nonumber
\\
&&+\frac{192\alpha^{2}\phi}{A\left(\chi,\phi\right)\chi}\left(\partial_{\left(\mu\right.}\chi\partial_{\left.\nu\right)}\phi-\frac{1}{2}g_{\mu\nu}\partial_{\rho}\chi\partial^{\rho}\phi\right)+\frac{1}{2}g_{\mu\nu}\frac{\mathcal{U}\left(\chi,\phi\right)}{\chi},
\end{eqnarray}
where the explicit expressions of $\mathcal{U}\left(\chi,\phi\right)$, $M_{T}^{2}\left(\chi\right)$ and $M_{S}^{2}\left(\chi\right)$ are given in Eq. \eqref{biscalarfunctions}, and 
\begin{equation}
A\left(\chi,\phi\right)=4\left[(4\alpha\phi)^{2}-9M_{S}^{2}(\chi)M_{T}^{2}(\chi)\right].
\end{equation}
It is also worth calculating the trace of Eq. \eqref{biscalar:Einstein}, which is given by
\begin{eqnarray}
\label{biscalar:Einsteintrace}
\mathring{R}&=&-\frac{72M_{S}^{2}\left(\chi\right)}{A\left(\chi,\phi\right)\chi}\partial_{\rho}\chi\partial^{\rho}\chi+\frac{3}{\chi}\Box\chi-\frac{72\alpha^{2}M_{T}^{2}\left(\chi\right)}{A\left(\chi,\phi\right)\chi}\partial_{\rho}\phi\partial^{\rho}\phi
\nonumber
\\
&&+\frac{192\alpha^{2}\phi}{A\left(\chi,\phi\right)\chi}\partial_{\rho}\chi\partial^{\rho}\phi-4\frac{\mathcal{U}\left(\chi,\phi\right)}{\chi}.
\end{eqnarray}

\item Variations with respect to the scalar $\chi$:
\begin{equation}
\frac{\delta S}{\delta\chi}=0\Longrightarrow\frac{\partial\mathcal{L}}{\partial\chi}-\partial_{\mu}\left(\frac{\partial\mathcal{L}}{\partial\left(\partial_{\mu}\chi\right)}\right)=0.
\end{equation}
Therefore we obtain
\begin{eqnarray}
\label{biscalar:chieq}
\mathring{R}&=&-\frac{a_{0}-\chi}{b_{1}}+\frac{144M_{S}^{2}\left(\chi\right)}{A\left(\chi,\phi\right)}\Box\chi-24\frac{\left(12M_{S}^{2}\left(\chi\right)\right)^{2}-\left(4\alpha\phi\right)^{2}}{A\left(\chi,\phi\right)^{2}}\partial_{\rho}\chi\partial^{\rho}\chi
\nonumber
\\
&&-\frac{192\alpha^{2}\phi}{A\left(\chi,\phi\right)}\Box\phi-72\alpha^{2}\frac{3M_{T}^{2}\left(\chi\right)\left(M_{T}^{2}\left(\chi\right)-20M_{S}^{2}\left(\chi\right)\right)-320\alpha^{2}\phi^{2}}{A\left(\chi,\phi\right)^{2}}\partial_{\rho}\phi\partial^{\rho}\phi
\nonumber
\\
&&-\frac{18432\alpha^{2}M_{S}^{2}\left(\chi\right)}{A\left(\chi,\phi\right)^{2}}\partial_{\rho}\chi\partial^{\rho}\phi.
\end{eqnarray}
This expression can be written in terms of $\chi$ and $\phi$ exclusively by substituing the Ricci scalar using Eq. \eqref{biscalar:Einsteintrace}, namely
 \begin{eqnarray}
&&\overline{\mathcal{U}}\left(\chi,\phi\right)-3\left[48\chi M_{S}^{2}\left(\chi\right)-A\left(\chi,\phi\right)\right]\Box\chi
\nonumber
\\
&&+96\frac{27m_{T}^{2}\left(M_{S}^{2}\left(\chi\right)\right)^{2}-8\alpha^{2}\phi^{2}\left(6m_{S}^{2}+\chi\right)}{A\left(\chi,\phi\right)}\partial_{\rho}\chi\partial^{\rho}\chi+192\alpha^{2}\chi\phi\Box\phi
\nonumber
\\
&&+24\alpha^{2}\frac{H_1\left(\chi\right)-192\alpha^{2}\phi^{2}M_{T}^{2}\left(\chi\right)-768\alpha^{2}\chi\phi^{2}}{A\left(\chi,\phi\right)}\partial_{\rho}\phi\partial^{\rho}\phi
\nonumber
\\
&&+768\alpha\phi\frac{H_{2}\left(\chi\right)+32\alpha^{2}\phi^{2}}{A\left(\chi,\phi\right)}\partial_{\rho}\chi\partial^{\rho}\phi=0,
\end{eqnarray}
where
\begin{eqnarray}
&&\overline{\mathcal{U}}\left(\chi,\phi\right)=A\left(\chi,\phi\right)\left[\frac{a_{0}\left(a_{0}-\chi\right)}{2b_{1}}+2\alpha\phi^{2}\right],
\\
&&H_{1}\left(\chi\right)=36M_{S}^{2}\left(\chi\right)M_{T}^{2}\left(\chi\right)\left(3M_{T}^{2}\left(\chi\right)-8\chi\right)+\left(3M_{T}^{2}\left(\chi\right)\right)^{2}\chi,
\\
&&H_{2}\left(\chi\right)=9M_{S}^{2}\left(\chi\right)M_{T}^{2}\left(\chi\right)+48\chi M_{S}^{2}\left(\chi\right)-3\chi M_{T}^{2}\left(\chi\right)-4\chi^{2}.
\end{eqnarray}

\item Variations with respect to the pseudo-scalar $\phi$:
\begin{equation}
\frac{\delta S}{\delta\phi}=0\Longrightarrow\frac{\partial\mathcal{L}}{\partial\phi}-\partial_{\mu}\left(\frac{\partial\mathcal{L}}{\partial\left(\partial_{\mu}\phi\right)}\right)=0.
\end{equation}
Accordingly we get
\begin{eqnarray}
&&-2\alpha\phi A\left(\chi,\phi\right)+192\alpha^{2}\phi\Box\chi-\frac{576\alpha^{2}\left(32M_{S}^{2}\left(\chi\right)-M_{T}^{2}\left(\chi\right)\right)\phi}{A\left(\chi.\phi\right)}\partial_{\rho}\chi\partial^{\rho}\chi
\nonumber
\\
&&-144M_{T}^{2}\left(\chi\right)\Box\phi+\frac{\left(96\alpha^{2}\right)^{2}M_{T}^{2}\left(\chi\right)\phi}{A\left(\chi,\phi\right)}\partial_{\rho}\phi\partial^{\rho}\phi
\nonumber
\\
&&+\frac{48\alpha^{2}\left[\left(16\alpha\phi\right)^{2}-\left(3M_{T}^{2}\left(\chi\right)\right)^{2}\right]}{A\left(\chi,\phi\right)}\partial_{\rho}\chi\partial^{\rho}\phi=0.
\end{eqnarray}

\end{itemize}
